UAV Optimal Guidance in Wind Fields Using ZEM/ZEV with Generalized Performance Index

This paper presents an optimal guidance approach for a UAV navigation between two given points in 3D considering the wind influence. The proposed cost function to be minimized involves the weighting of the travel time and the control energy. An analytical expression is derived for the optimal cost yielding a fourth-order polynomial whose positive real roots correspond to the optimal travel times. The optimization problem is shown to be equivalent to the Zero-Effort-Miss/Zero-Effort-Velocity (ZEM/ZEV) optimal guidance approach for the case of a constant wind acceleration. Case studies for the rendez-vous and the intercept problems are shown through simulation examples for different wind conditions.

==> AnalysisPareto.tex <==
\section{Analysis of Pareto-Optimal (no wind case)}
\label{sec:analysispareto}

In this section, we develop some relations between the Pareto-Optimal
cuve and the case of multiple solutions for a same ``$C_{I}$''
trade-off parameter in the optimal trajectory control problem, recalling
that the Pareto-Optimal is a tradeoff curve between the total flight
time $t_{f}$ and the amount of control energy $\intop u^{T}u$ required
for different values of $C_{I}$.

A typical example of a Pareto-Optimal is the red curve in Figure 1
below, obtained for the case $x_{g0}=-4,\,v_{xg0}=-12,\,v_{yg0}=0$
and null wind condition ($W_{x}=0,\,W_{y}=0).$ This plot shows the
conflict that appears when one searches for the minimum travel time
$t_{f}$ and minimum energy at the same time.

%\selectlanguage{brazil}%
\begin{figure}
\noindent \begin{centering}
\includegraphics[scale=0.5]{figs/Paretos}
\par\end{centering}
\noindent \centering{}\caption{{Pareto-Optimal curves for ($x_{0}=4,\,v_{x0}=-12,\,v_{y0}=0)$ and
no wind, when there are 3 optimal solutions for $t_{f}$. }}
\end{figure}

%\selectlanguage{english}%
We can see from this plot that there are three main branches, corresponding
to the three positive real roots. The first branch (in blue) corresponds
to the lower positive real root that exhibits no reversal movement
(0<K<3), with $C_{I}$ allowed to vary in the range from 0 to infinty,
and with high energy consumption. The second branch (in black) corresponds
to the middle positive real root (with 3<K<6) and $C_{I}$ allowed
to vary in the range $0<C_{I}<15.$ The third branch (in red) is related
to the bigger positive real root with $C_{I}$ in the range $0<C_{I}<18$
and $t_{f}$ varying from $6t_{r}$ to infinty, and with low energy
consumption.

We will show, in the sequel, that all the critical values of time,
energy and $C_{I}$ in this figure can be derived analytically. An
interesting related result for ``LQR minimum-time problem'' showing
the same three critical points of K=0, K=3 and K=6 in a root locus
plot can be found in the reference (Verriest and Lewis, 1991), although
there is no analysis for the critical $C_{I}$ trade-off parameter.

We will show that the critical point of $C_{I}=18=\left(\dfrac{v_{xg0}^{4}}{72x_{g0}^{2}}\right)$
corresponding to the optimal final time $t_{f}=6t_{r}=6\left(-\dfrac{x_{g0}}{v_{xg0}}\right)$
in this figure is associated to one bifurcation point (see figure
7) when the roots of the quartic polynomial are changing from the
condition of ``3 positives and 1 negative real roots'' to ``two
complex roots, one positive root and one negative root''. 

%\selectlanguage{brazil}%
\begin{figure}
\noindent \begin{centering}
\includegraphics[scale=0.46]{figs/Paretos_CIb}
\par\end{centering}
\noindent \centering{}\caption{Roots of optimal polynomial for the same case, and for 3 different
$C_{I}$ parameters. }
\end{figure}

%\selectlanguage{english}%
We present, in the sequel, the analytical developments for the derivation
of these ``critical'' values.

Firstly, we recall the quartic polynomial equation for the optimal
$t_{f}$ (Carvalho, 2018), with $v_{yg0}=0$ and $W_{x}=0$ is reduced
to
\[
C_{I}t_{f}^{4}-2(v_{xg0}^{2})t_{f}^{2}-12(v_{xg0}x_{g0})t_{f}-18(x_{g0}^{2})=0
\]

As well as the equations of the optimal velocity and optimal acceleration
\[
\begin{array}{c}
v_{xg}(t)=\dfrac{J_{x}t^{2}}{2}-J_{v_{x0}}t+v_{xg0}\\
u(t)=-J_{x}t+J_{v_{x0}}
\end{array}
\]

where the costates are given by
\[
J_{x}=\dfrac{6(2x_{g0}+v_{xg0}t_{f})}{t_{f}^{3}},\,\,\,\,\,\,\,\,\,\,J_{vx0}=\dfrac{2(3x_{g0}+2v_{xg0}t_{f})}{t_{f}^{2}}
\]

As presented in (Carvalho, 2018), an alternative equation for the
optimal acceleration is given by
\begin{equation}
u(t)=-J_{vx}=\sqrt{2C_{I}+2J_{x}v_{x}(t)}\label{eq:u_opt}
\end{equation}

As we know that the final velocity $v_{xg}(t_{f})$ should be null,
we can look for an explicit equation for the roots of the quadratic
function $v_{xg}(t)$ as
\[
t_{v1,v2}=\dfrac{J_{vx0}\pm\sqrt{J_{vx0}^{2}-2J_{x}v_{0}}}{J_{x}}
\]

Where we used the subscript ``v'' to distinguish the roots of the
quadratic velocity polynomial from the roots of the quartic polynomial
(although some of the roots of the quartic polynomial will also be
roots of the quadratic velocity polynomial). From the acceleration
equation in (\ref{eq:u_opt}) we have that $J_{vx0}^{2}=u_{0}^{2}$
and $2C_{I}=J_{vx0}^{2}-2J_{x}v_{xg0}$, and thus the two roots of
the velocity equation can be written as
\[
t_{v1,v2}=\dfrac{J_{vx0}\pm\sqrt{2C_{I}}}{J_{x}}
\]

Look that the middle point between these two roots occur in the time
instant $t=\dfrac{J_{vx0}}{J_{x}}$ that is exactly the point where
the acceleration is null.

As we know that in the critical point of the bifurcation we have the
critical value of K=6, and with the relations obtained previously
for the gains of the quartic polynomial in the bifurcation point as

\[
\left\{ \begin{array}{ccc}
k_{0}=K^{2}\dfrac{x_{g0}^{2}}{v_{x0}^{2}} & \,\,\,\,\,\, & k_{1}=\dfrac{18v_{xg0}^{2}}{C_{I}K^{2}}\end{array}\right.
\]

then we have a simple relation for the ``critical'' $C_{I}$ as
\[
C_{I}=\dfrac{v_{xg0}^{4}}{72x_{g0}^{2}}
\]

Now, with this critical value of $C_{I}$ and knowing that $t_{f}=6t_{r}=6\left(-\dfrac{x_{0}}{v_{0}}\right)$,
we can check for the second root of the quadratic polynomial of the
velocity equation:
\[
t_{v1,v2}=\dfrac{J_{vx0}\pm\sqrt{2C_{I}}}{J_{x}}=\dfrac{J_{vx0}\pm\sqrt{\dfrac{v_{0}^{4}}{36x_{0}^{2}}}}{J_{x}}=\dfrac{J_{vx0}\pm\dfrac{v_{0}^{2}}{6x_{0}}}{J_{x}}
\]

Or
\[
t_{v1,v2}=\dfrac{\dfrac{2(3x_{g0}+2v_{xg0}t_{f})}{t_{f}^{2}}\pm\dfrac{v_{0}^{2}}{6x_{0}}}{\dfrac{6(2x_{g0}+v_{xg0}t_{f})}{t_{f}^{3}}}=\dfrac{2(3x_{g0}+2v_{xg0}t_{f})t_{f}\pm\dfrac{v_{0}^{2}}{6x_{0}}t_{f}^{3}}{6(2x_{g0}+v_{xg0}t_{f})}
\]

Or
\[
t_{v1,v2}=\dfrac{2(3x_{g0}+12v_{xg0}t_{r})t_{f}\pm\dfrac{v_{0}^{2}}{6x_{0}}t_{f}^{3}}{6(2x_{g0}+6v_{xg0}t_{r})}=\dfrac{2(-9x_{g0})t_{f}\pm\dfrac{v_{0}^{2}}{6x_{0}}t_{f}^{3}}{6(-4x_{g0})}
\]

Or

\[
t_{v1,v2}=\dfrac{2(-9x_{g0})t_{f}\pm\dfrac{v_{0}^{2}}{6x_{0}}t_{f}^{3}}{6(-4x_{g0})}=\dfrac{2(-9x_{g0})(6t_{r})\pm\dfrac{v_{0}^{2}}{6x_{0}}(6t_{r})^{3}}{6(-4x_{g0})}
\]

Or finally

\[
t_{v1,v2}=\dfrac{2(-9x_{g0})(6t_{r})\pm\dfrac{v_{0}^{2}}{6x_{0}}(6t_{r})^{3}}{6(-4x_{g0})}=4.5t_{r}\pm1.5t_{r}
\]

Which confirms that for the critical $C_{I}$, the two roots of the
quadratic velocity equation (for $t_{f}=t_{4}$ coming from the quartic
polynomial) are $t_{v1}=3t_{r}$ and $t_{v2}=6t_{r}.$ And as we have
seen previously that the notable value of $t_{f}=3t_{r}$ is an optimal
solution for this problem only when $C_{I}=0,$ then we conclude that
$t_{v2}=6t_{r},$ that is indeed a double root ($t_{3}=t_{4})$ of
the quartic polynomial with critical $C_{I}$, is the only possible
solution from these two roots for the quadratic polynomial. The other
optimal solution of the quartic polynomial, in this critical $C_{I}$
case, comes from ($t_{2})$. The figure below illustrate these relations
on the roots for the critical case ($C_{I}=C_{I,critic})$, while
the other figure in the sequel illustrates the general case ($C_{I}<C_{I,critic}).$

%\selectlanguage{brazil}%
\begin{figure}
\noindent \begin{centering}
\includegraphics[scale=0.52]{figs/Pareto3_CI_18b}
\par\end{centering}
\noindent \centering{}\caption{{Optimal acceleration, velocity and position responses for $C_{I}=18$.
The 3 positive real solutions of the time polynomial degenerate to
2 solutions, as $t_{3}=t_{4}$ is a double root. Note that the ``yellow''
root is a root of the quadratic velocity polynomial for $t_{f}=6t_{r}$
but it is not a root of the optimal quartic polynomial in $t_{f.}$}}
\end{figure}


==> LQR.tex <==
\section{Relations with the LQR Minimum Time Problem (LQR-MT)}
\label{sec:lqr}

An interesting relation between bifurcations \cite{2004Bif} and the root locus plots for the quartic time polynomial can be traced. 

The classical paper of Frank Lewis \cite{Lewis1991} investigates a nontraditional minimum-time problem that includes quadratic state and control weighting terms in the performance index that can be shown to be equivalent, in some cases, to the same problem presented here for the "no wind" case. Although this problem has been investigated since the 1960's, in \cite{Lewis1991} it was fully exploited, by the first time with a formal analytic solution, yielding a convenient and practical design technique that is used still today in autonomous vehicle control \cite{2017Kumar}.

\begin{figure}[hbt]
\noindent \begin{centering}
\includegraphics[scale=0.66]{figs/rlocusT.png}
\par\end{centering}
\noindent \centering{}\caption{Root locus of $t_f$ as function of $\frac{1}{C_I}$ for the quartic polynomial with a given $x_g0$ and $v_{xg0}$: (a) $W_x=0$ in black and $W_x=v_{xg0}$ in red; (b) $W_x=0, \frac{1}{3}, \frac{2}{3}$ and $\frac{3}{3}$ of $v_{xg0}$; (c) $W_x=v_{xg0}$ in black and $W_x=4v_{xg0}$ in red.}
\label{fig:rootlocus}
\end{figure}

In their work, the authors show that the roots of the optimal polynomial (\ref{eq:tf}) for the X-longitudinal movement with a given initial velocity $v_{xg0}$ and no wind ($W_x=W_y=0$) can be represented in a root locus plot, where the gain $\rho=\frac{1}{C_I}$ varies from 0 to infinity. This root locus is shown in the upper part of Figure \ref{fig:rootlocus} by the red circle and the real axis. The open loop transfer in this root locus plot has four poles at the origin and two zeros at the center of the circle ($z=3t_r=-3\frac{x_0}{v_{xg0}}$).

Note that these plots show the roots of the optimal polynomial as function of the trade-off parameter $C_I$ (indeed $\frac{1}{C_I}$), for a given fixed $v_{xg0}$. Instead, the curves used in our paper to derive the bifurcation points (as in the right side of this same figure \ref{fig:rootlocus}) show the roots of the same polynomial as function of $v_{xg0}$, for a given fixed $C_I$. Thus, for the "no wind" case, we can give a new interpretation of the root locus analysis of \cite{Lewis1991}, where the two bifurcation points ($K=6$ and $K=3$) will be represented, respectively by the zeros at $3t_r$ and the branch interception point at $6t_r$. One can understand the "evolution" of the roots locus, as the gain varies from 0 to infinity ($C_I$ varying from infinity to zero), if you select a fixed initial velocity $\bar{v}_1$ (figure \ref{fig:rootlocus} up-right) and "observe" the number of real roots crossing the vertical line at $\bar{v}_1$, while the different plots (for different $C_I$) are "moving" from the left to the right.

Now, if we assume the "with wind" case, a similar conclusion can be drawn. For the particular case of $v_{xg0}=W_x$, the resulting root locus is the black circle in Figure \ref{fig:rootlocus} (a). Look that now, the two bifurcation points are $K=1.5t_r$ and $K=3t_r$. The same root locus plots can be traced for $v_{xg0}<W_x$ (see $\bar{v}_2$ in figure \ref{fig:rootlocus}-b) and $v_{xg0}>W_x$ (see $\bar{v}_3$ in figure \ref{fig:rootlocus}-c). Look that the plots also confirm that there is always one positive real root in all situations.



==> PracticalAspects.tex <==
\section{Practical Implementation Considerations}
\label{sec:casestudies}
We present here four main case 


\begin{figure}[h]
\noindent \begin{centering}
\includegraphics[scale=0.2]{figs/exemplo4D.png}
\par\end{centering}
\noindent \centering{}\caption{Optimal final time (in K) and paths for $x_{g0}=40$, $v_{yg0}=-4$, $C_I=1$, for 3 wind values:  $W_x=-2$ (red), $W_x=+2$ (blue), $W_x=0$ (black), and for two longitudinal speeds $v_{xg0}=-6$ and $v_{xg0}=-12$.  Plot steps of 0.2 sec.} 
\label{fig:caso4}
\end{figure}

==> Preliminaries.tex <==
\section{Preliminary definitions}
\label{sec:preliminaries}

Prior to analyse the solution of the optimization problem for some
particular wind cases, it is important, first, to present the physical
interpretations of the optimal velocity-acceleration responses for
some special cases of $t_{f}$ - roots of the optimal polynomial in
(\ref{eq:polygeral}) - as function of $x_{0,}v_{x0}.$ We consider here
$x_{0}v_{x0}<0,$ that is the usual case of a initial velocity
pointing toward the target. For this purpose, let us define a constant
$t_{r}$, denoted as ``reference time'', or $t_{r}=-\dfrac{x_{g0}}{v_{xg0}}$,
such that the final time can be written as a multiple of this reference
time, or $t_{f}=-K\dfrac{x_{g0}}{v_{xg0}}=Kt_{r}.$

The physical interpretation for the velocity-acceleration responses
for $K=1,2,3$ is resumed in Table 1.

~

\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline 
$K^*$ & position & velocity & acceleration\tabularnewline
\hline 
\hline 
1 & linear, with $x(t_{f})=0$ & constant, such that $v_{x}(t_{f})\neq0$ & null\tabularnewline
\hline 
2 & quadratic, with x($t_{f})=0$ & linear, with $v_{x}(t_{f})=0$ & constant for $K^*=2$ \tabularnewline
& &  & crescent for $K^*<2$ \tabularnewline
& &  & decrescent for $K^*>2$ \tabularnewline
\hline 
3 & cubic, with x($t_{f})=0$ & quadratic, with $v_{x}(t_{f})=0$ and $v_{xg0}v_{x}(t_{f}^{-})>0$  & linear and $\dot{v}_{x}(t_{f})=0$\tabularnewline
\hline 
>3 & cubic, with x($t_{f})=0$ & quadratic, with $v_{x}(t_{f})=0$ and $v_{xg0}v_{x}(t_{f}^{-})<0$ & linear and $\dot{v}_{x}(t_{f})\neq0$\tabularnewline
\hline 
\end{tabular}
\end{center}
\begin{center}
Table 1 - Physical interpretation for the time responses when $K^*=1,2,3$ and when $K^*>3.$
\end{center}

\begin{figure}
\noindent \begin{centering}
\includegraphics[scale=0.48]{figs/Br_physical}
\par\end{centering}
\noindent \centering{}\caption{Accelerations (red), velocities (blue) and positions (black) for{
$(x_{0},v_{x0})=(4,-12)$ in four special cases of $t=-t_{r,}-2t_{r,}-3t_{r}$
and} {$t_{f}=-10t_{r}$}.}
\end{figure}


Obviously K=1 will never be a solution for the rendezvous case with null terminal velocity, as $v_{x}(t_{f})\neq0$.
However, K=2 may be an optimal solution of ``degenerated type''
as in this case the optimal acceleration will be constant. Another
interesting point is that if K<2, then the linear acceleration is
a decrescent function, and for K>2 the acceleration is a crescent
function. It is interesting to note also that the solution with K=3
is the only possible optimal case in wich the final acceleration is
null, or $\dot{v}_{x}(t_{f})=0.$ Figure 2 illustrates these 3 special
situations for the particular case of $(x_{0},v_{x0})=(4,-12)$, as
well as a fourth one, illustrating the situation when K>3. Indeed,
it is possible to show {[}Guo, 2013{]} that whenever $K>3$, a reversal
movement in the X-displacement will occur, with a change of sign in
the velocity curve during the movement, as illustrated in Figure 3.
This backward movement for K>3 will occur independent of the Y-response,
as the responses in each dimension are decoupled (coupled only through
 $t_{f}$). 

==> discussion_old.tex <==
\section{On the existence of solutions for the minimum control energy case}
\label{seven}

It has already been proved that the general depressed quartic time-optimal polynomial in (\ref{eq:polygeral}) has always at least one positive real root \cite{DSouza1997}, \cite{Carvalho2018}.
However, in the particular case of $C_I=0$, then the quartic polynomial degrades to a second order polynomial that may not admit a positive real root in some cases.

The existence of a feasible solution for this minimum energy problem $(C_I=0)$ is discussed in \cite{Guo2019}, where a trade-off cost function is introduced in the ZEM/ZEV approach for orbital intercept/rendezvous.
In their case, the Hamiltonian equation is very similar to (\ref{eq:Ham}), while they have the gravity vector in place of the wind acceleration vector of our case.

According to the authors in \cite{Guo2019}, one possible explanation for the inexistence of solutions is that, with $C_I=0$, the terminal time is neither constrained nor penalized and, in this way, a longer $t_f$ yields a smaller cost-to-go, and no finite $t_f$ would minimize the integral of energy. %Also, the authors considers this an "interesting subject for further study".
Although this makes sense, it does not explain, however, why there are some cases in which  $C_I=0$ yields a finite positive terminal time, as we show in the sequel. In other words, in some situations, there exists a finite $t_f$ minimizing the integral of control energy, as a local optimum solution.
Aiming a better comprehension for this behavior in the time solutions, we investigate here two special cases, under a constant wind.

Consider the problem, shown in Figure 9, for a 2D path, with $y_0=0$, $C_I=0$ and ${\bf k=0}$,  for both rendezvous/intercept, where one wants to find the maximum initial heading $\theta$ for which a finite terminal time $t_f$ exists. For the rendezvous, we assume $v_{xf}=v_{x0}$,$v_{yf}=-v_{y0}$, and for the intercept, the terminal velocities  are free at the target. Such that the problem can be translated into one that searches for the maximum  allowable $v_{y0}$, for a given $v_{x0}$.

\begin{figure}[hb]
\noindent \begin{centering}
\includegraphics[scale=0.60]{figs/AIAA_fig_wind_heading.png}
\par\end{centering}
\noindent \centering{}\caption{{Search for the maximum initial heading $\theta$, with $C_I=0$, to obtain a finite optimal $t_f$ solution.}}
\end{figure}

The corresponding optimal-time polynomials, using (\ref{eq:polyrendezvous}) and (\ref{eq:poly_Inter}) for both optimal problems are:

%\begin{equation}
%\begin{array}{l}
%  \mbox{Rendezvous}~~~~~   P(t_{f})=2C_{I}t_{f}^{4}-4(3v_{gx0}^{2}+v_{gy0}^{2})t_{f}^{2}-48{\bf r_{0}}^{T}{\bf v}_{g0}t_{f}-36{\bf r_{0}}{}^{T}{\bf r_{0}} \\
%    \mbox{Intercept}~~~~~~~~~~
%P(t_{f})=2C_{I}t_{f}^{4}-3{\bf v}_{g0}{}^{T}{\bf v}_{g0}t_{f}^{2}-12{\bf r_{0}}^{T}{\bf v}_{g0}t_{f}-9{\bf r_{0}}{}^{T}{\bf r_{0}} \\
%\end{array}
%\end{equation}

%Which, with the given initial/terminal velocities, can be rewritten as:

\begin{equation}
\begin{array}{l}
 \mbox{Rendezvous}~~~~~   \\
 
P(t_{f})=(2C_{I}+{\bf k}^{T}{\bf k})t_{f}^{4}
-4({\bf v}_{g0}{}^{T}{\bf v}_{g0}+{\bf v}_{gf}{}^{T}{\bf v}_{gf}+{\bf v}_{gf}^{T}{\bf v}_{g0})t_{f}^{2}
-24{\bf r_{0}}^{T}({\bf v}_{g0}+{\bf v}_{gf})t_{f}-36{\bf r_{0}}{}^{T}{\bf r_{0}}\\

P(t_{f})=2C_{I}t_{f}^{4}
-4({\bf v}_{g0}{}^{T}{\bf v}_{g0}+{\bf v}_{gf}{}^{T}{\bf v}_{gf}+{\bf v}_{gf}^{T}{\bf v}_{g0})t_{f}^{2}
-24{\bf r_{0}}^{T}({\bf v}_{g0}+{\bf v}_{gf})t_{f}-36{\bf r_{0}}{}^{T}{\bf r_{0}}\\

P(t_{f})=2C_{I}t_{f}^{4}
-4(3v_{gx0}^{2}+v_{gy0}^{2})t_{f}^{2}
-24{\bf r_{0}}^{T}({\bf v}_{g0}+{\bf v}_{gf})t_{f}-36{\bf r_{0}}{}^{T}{\bf r_{0}}\\

P(t_{f})=2C_{I}t_{f}^{4}
-4(3v_{gx0}^{2}+v_{gy0}^{2})t_{f}^{2}
-48(x_{0}v_{gx0})t_{f}-36x_{0}^{2}\\ \\

  \mbox{Intercept}~~~~~~~~~~\\
  
  P(t_{f})=2C_{I}t_{f}^{4}-3{\bf v}_{g0}{}^{T}{\bf v}_{g0}t_{f}^{2}-12{\bf r_{0}}^{T}{\bf v}_{g0}t_{f}-9{\bf r_{0}}{}^{T}{\bf r_{0}}\\
  
  P(t_{f})=2C_{I}t_{f}^{4}-3(v_{gx0}^{2}+v_{gy0}^{2})t_{f}^{2}-12(x_{0}v_{gx0})t_{f}-9x_{0}^{2}=0 \\
  \label{eq:poly_compara}
\end{array}
\end{equation}

\begin{equation}
\begin{array}{l}
 \mbox{Rendezvous}~~~~~     P(t_{f})/4=(\dfrac{C_{I}}{2})t_{f}^{4}-(3v_{gx0}^{2}+v_{gy0}^{2})t_{f}^{2}-12(x_{0}v_{gx0})t_{f}-9x_{0}^{2} \\
  \mbox{Intercept}~~~~~~~~~~
  P(t_{f})=2C_{I}t_{f}^{4}-3(v_{gx0}^{2}+v_{gy0}^{2})t_{f}^{2}-12(x_{0}v_{gx0})t_{f}-9x_{0}^{2} \\
  \label{eq:poly_compara}
\end{array}
\end{equation}

\indent And if we consider $C_I=0$, then both polynomials will be very similar. 

\begin{equation}
\begin{array}{l}
 \mbox{Rendezvous}~~~~~     P(t_{f})/4=0\to-(3v_{gx0}^{2}+v_{gy0}^{2})t_{f}^{2}-12(x_{0}v_{gx0})t_{f}-9x_{0}^{2}=0 \\
  \mbox{Intercept}~~~~~~~~~~
  P(t_{f})=0\to-3(v_{gx0}^{2}+v_{gy0}^{2})t_{f}^{2}-12(x_{0}v_{gx0})t_{f}-9x_{0}^{2}=0 \\
  \label{eq:poly_compara}
\end{array}
\end{equation}

And if we write the terminal time $t_f$ as a function of the reference time (Table 1), or $t_{f}=Kt_{r}=K\left( -\frac{x_{g0}}{v_{xg0}} \right)$, we have

\begin{equation}
\begin{array}{l}
 \mbox{Rendezvous}~~~~~     P(t_{f})/4=0\to-(3v_{gx0}^{2}+v_{gy0}^{2})K^{2}\left( -\frac{x_{g0}}{v_{xg0}} \right)^{2}-12(x_{0}v_{gx0})K\left( -\frac{x_{g0}}{v_{xg0}} \right)-9x_{0}^{2}=0 \\
  \mbox{Intercept}~~~~~~~~~~
  P(t_{f})=0\to-3(v_{gx0}^{2}+v_{gy0}^{2})K^{2}\left( -\frac{x_{g0}}{v_{xg0}} \right)^{2}-12(x_{0}v_{gx0})K\left( -\frac{x_{g0}}{v_{xg0}} \right)-9x_{0}^{2}=0 \\
  \label{eq:poly_compara}
\end{array}
\end{equation}

\begin{equation}
\begin{array}{l}
 \mbox{Rendezvous}~~~~~    
  P(t_{f})=0\to
  \left(\dfrac{-3(v_{gx0}^{2}+\frac{1}{3}v_{gy0}^{2})}{v_{gx0}^{2}}\right)
  K^{2}x_{0}^{2}+12Kx_{0}^{2}-9x_{0}^{2}=0\\
  \mbox{Intercept}~~~~~~~~~~
  P(t_{f})=0\to
  \left(\dfrac{-3(v_{gx0}^{2}+v_{gy0}^{2})}{v_{gx0}^{2}}\right)
  K^{2}x_{0}^{2}+12Kx_{0}^{2}-9x_{0}^{2}=0 \\
  \label{eq:poly_compara}
\end{array}
\end{equation}

\begin{equation}
\begin{array}{l}
 \mbox{Rendezvous}~~~~~    
  P(t_{f})=0\to
  \left(\dfrac{-3(v_{gx0}^{2}+\frac{1}{3}v_{gy0}^{2})}{v_{gx0}^{2}}\right)
  K^{2}+12K-9=0\\
  \mbox{Intercept}~~~~~~~~~~
  P(t_{f})=0\to
  \left(\dfrac{-3(v_{gx0}^{2}+v_{gy0}^{2})}{v_{gx0}^{2}}\right)
  K^{2}+12K-9=0 \\
  \label{eq:poly_compara}
\end{array}
\end{equation}

\begin{equation}
\begin{array}{l}
 \mbox{Rendezvous}~~~~~    
  P(t_{f})=0\to
 \alpha_{0R}
  K^{2}+12K-9=0\\
  \mbox{Intercept}~~~~~~~~~~
  P(t_{f})=0\to
  \alpha_{0I}
  K^{2}+12K-9=0 \\
  \label{eq:poly_compara}
\end{array}
\end{equation}

And in both cases above, for the critical (double) root, for which the discrimant of the simplified quadratic polynomial is null, the highest degree coefficient, $\alpha_0$, should be equal to -4, such that we have:

\begin{equation}
\begin{array}{c}
      P(K)=(\alpha_0) K^{2}+12K-9=0  \\ 
    P(K)=-4 K^{2}+12K-9=0  \\ 
    K=1.5 \\ \\
  
   \mbox{~~Rendezvous} ~~~~~~~~~~~~~~~~~~~~~~~~~~\mbox{~~~ ~~~Intercept}\\
   
   \alpha_{0R}=\left( \dfrac{-3( v_{gx0}^{2}+\frac{1}{3}v_{gy0}^{2})}{v_{gx0}^{2} }\right)=-4 ~~~~~~
   \alpha_{0I}=\left(\dfrac{-3(v_{gx0}^{2}+v_{gy0}^{2})}{v_{gx0}^{2}}\right)=-4  \\
\end{array}
\end{equation}

While the corresponding critical orthogonal velocity, and the maximum initial heading for each case are:

\begin{equation}
\begin{array}{l}
 \mbox{Rendezvous}~~~~~       v_{{gy0}_{MAX}}=v_{gx0}~~~~~~~~~\theta_{MAX}=45~ deg \\ 
  \mbox{Intercept}~~~~~~~~~~
v_{{gy0}_{MAX}}=\dfrac{v_{gx0}}{\sqrt{3}}~~~~~~~~\theta_{MAX}=30 ~deg\\
\end{array}
\end{equation}

The heading limitation ($30 ~deg$) for the intercept problem is in agreement with the results of \cite{Hawking2013}, although there was not a corresponding analysis for the rendezvous case.\textcolor{red}{ Maybe because in this case, the maximum initial heading will depend on the value of the final velocity. Note that we considered here the case  $v_{xf}=v_{x0}$,$v_{yf}=-v_{y0}$. When the final velocity is NULL, the maximum initial heading for the Rendezvous problem is zero (only the straight direction will yield a feasible solution), as will be shown
in the simulation example of the next section.}
Note also that in  \cite{Bakolas2014} there is no initial heading constraint for the optimal intercept, as they work with a minimum-time problem.

A plot of the optimal $K$-parameter (multiple of the reference time) as function of the orthogonal velocity $v_{gy0}$, for a problem with $x_0=3,v_{gx0}=-1$ is shown in Figure 10-right, for both cases.
\begin{figure}[hbtp]
\noindent \begin{centering}
\includegraphics[scale=0.68]{figs/roots_intercept2c.png}
\par\end{centering}
\noindent \centering{}\caption{{Roots of time-optimal polynomial as function of $v_{gyo}$, with $C_I=1e^{-6},x_0=3,v_{gx0}=-1.$}}
\end{figure}
Now, if instead of working with the simplified quadratic polynomials (with $C_I=0$), we work with the original quartic polynomial in (\ref{eq:poly_compara}), with a very small $C_I$, then we have the plot of the $K$-parameter as shown in Figure 10-left. Note that we show, in this figure, only the 3 positive real roots of the polynomial (as the fourth one is negative), and notice also that we have always a large time solution, as $t_f \to \infty$ for $C_I \to 0$. This slow time response is the solution for the minimum-energy problem commented in \cite{Guo2019}, and it will always exists for any problem with $C_I \to 0$. But in some cases, there will still be other two local optimal time solutions. Indeed, this behavior in the multiple roots of a polynomial is known as "bifurcation", and was cited in  \cite{Bakolas2014}, for an intercept problem, as "jump solutions" or "manifold discontinuities". Note also that, although the intercept guidance in \cite{Bakolas2014} does not show heading constraints, it still may exhibit "jump solutions" corresponding to the point, or parameter, for which the number of positive real roots of $P(t_f)$ changes from 3 to 1.


\iffalse
\begin{table}
\caption{Cases of time-optimal polynomial $P(t_f)$}
\label{table:tablepoly}
\centering
\begin{tabular}{|c|c|c|c|}
\hline 
 Case & ${\bf v}_g(t_f)$  & $\frac{dw}{dt}$ & Polynomial $P(t_{f})$
 \tabularnewline
\hline 
\hline 
1 (R) & ${\bf 0}$ & ${\bf 0}$ & $C_{I}t_{f}^{4}-2({\bf v}_{g0}^{T}{\bf v}_{g0})t_{f}^{2}-12({\bf r_{0}}^{T}{\bf v}_{g0})t_{f}-18({\bf r_{0}}{}^{T}{\bf r_{0}})$
\tabularnewline
\hline 
2 (R) & ${\bf 0}$ & ${\bf {k}}$ &
$(2C_{I}+{\bf k}^{T}{\bf k})t_{f}^{4}-4({\bf v}_{g0}^{T}{\bf v}_{g0})t_{f}^{2}-24({\bf r_{0}}^{T}{\bf v}_{g0})t_{f}-36({\bf r_{0}}{}^{T}{\bf r_{0}})$
\tabularnewline
\hline 
3 (R) & ${\bf v}_{gf}$ & ${\bf \overline{k}}$ &
$(2C_{I}+{\bf \overline{k}}^{T}{\bf \overline{k}})t_{f}^{4}-4({\bf v}_{g0}{}^{T}{\bf v}_{g0}+{\bf v}_{gf}{}^{T}{\bf v}_{gf}+{\bf v}_{gf}^{T}{\bf v}_{g0})t_{f}^{2}-24{\bf r_{0}}^{T}({\bf v}_{g0}+{\bf v}_{gf})t_{f}-36{\bf r_{0}}{}^{T}{\bf r_{0}}$
\tabularnewline
\hline 
4 (R) & $[{\bf v}_{gx0},-{\bf v}_{gy0}]$
& ${\bf \overline{k}}$ &
$(2C_{I}+{\bf \overline{k}}^{T}{\bf \overline{k}})t_{f}^{4}-4(3v_{gx0}^{2}+v_{gy0}^{2})t_{f}^{2}-48{\bf r_{0}}^{T}{\bf v}_{g0}t_{f}-36{\bf r_{0}}{}^{T}{\bf r_{0}} $
\tabularnewline
\hline 
5 (R) & $[{\bf v}_{gx0},{\bf v}_{gy0}]$
& ${\bf \overline{k}}$ &
$(2C_{I}+{\bf \overline{k}}^{T}{\bf \overline{k}})t_{f}^{4}-12(v_{gx0}^{2}+v_{gy0}^{2})t_{f}^{2}-48{\bf r_{0}}^{T}{\bf v}_{g0}t_{f}-36{\bf r_{0}}{}^{T}{\bf r_{0}} $
\tabularnewline
\hline 
6 (I) &  free & ${\bf {k}}$ &
$(2C_{I}+\frac{3}{4}{\bf k}^{T}{\bf k})t_{f}^{4}-3({\bf v}_{g0}{}^{T}{\bf v}_{g0}+{\bf r_{0}}^{T}{\bf k})t_{f}^{2}-12{\bf r_{0}}^{T}{\bf v}_{g0}t_{f}-9{\bf r_{0}}{}^{T}{\bf r_{0}}$
\tabularnewline
\hline 
7 (I) & free &  ${\bf {0}}$ &
$2C_{I}t_{f}^{4}-3{\bf v}_{g0}{}^{T}{\bf v}_{g0}t_{f}^{2}-12{\bf r_{0}}^{T}{\bf v}_{g0}t_{f}-9{\bf r_{0}}{}^{T}{\bf r_{0}}$
\tabularnewline
\hline 
\end{tabular}
\end{table}
\fi


%It is interesting to note that, for a constant wind condition (${\bf k=0})$ and a minimum-energy problem $(C_{I}\to0),$ this quartic polynomial will be reduced to a 2nd order polynomial, which yields a positive real root only if $|v_{gy0}|\leq|v_{gx0}|,$ corresponding to an initial heading angle, toward the target, lesser than 45 deg. However, the inclusion of a trade-off paramenter $C_{I}\neq0$, or even the presence of a wind gradient ${\bf k \neq0}$, will withdraw this initial heading constraint, assuring at least one positive real root for the quartic polynomial, independent of the initial heading.



==> figs/discussionnew.tex <==
\section{Solutions for the minimum control energy case}
\label{sec:discussion}

Prior to analyzing the solution of the optimization problem for some
particular wind cases, it is important to present the physical
interpretations of the roots of the polynomial (\ref{polynomial}) as a function of $x_{0}$ and $v_{xg0}.$ 
Note that we consider here only the $x$-coordinate because we assumed that the target inertial frame is selected so that $y_0=z_0=0$.
We define a reference time-constant as
\begin{equation}\label{tr}
t_{r}=-\dfrac{x_{0}}{v_{xg0}}
\end{equation}
where  we assume that $x_{0}v_{xg0}<0$ so that the initial ground velocity in the x-coordinate is pointing toward $x=0$, which is considered to be the target point for the coordinate $x$.
The final time can then always be written as $t_{f}=Kt_{r}$ for an appropriate constant $K$.
The physical interpretation for the velocity-acceleration responses
for $K=1,1.5,2,3$ is summarized in Table 1.
Figure \ref{Figure3} illustrates the trajectories in $x$ for $K=1,1.5,2,3,$ and $K>3$ for $(x_{0},v_{x0})=(4,-12)$. 
It is possible to show that whenever $K>3$, a reversal
movement in the x-axis will occur \cite{Guo2012} with a change of sign in
the velocity curve during the movement, as illustrated in Figure 3 for the case $t_f=10t_{r}$.
The special case of $K=1.5$ will be further analysed in section VIII.

%Obviously $K=1$ will never be a solution for the rendezvous case with zero terminal velocity, as $v_{x}(t_{f})\neq0$.
%Note that $K=2$ is an optimal solution of ``degenerated type'',
%as in this case the optimal  polynomials  ($x,v_x,\dot{v}_x)$ show a decreased degree in order.
%Another interesting point is that if K<2, then the linear acceleration is a decrescent function, and for K>2 the acceleration is a crescent function. 
%It is interesting to note also that the solution with $K=3$
%is the only optimal case in which the final acceleration is
%zero, or $\dot{v}_{x}(t_{f})=0.$
%This backward movement for K>3 will occur independent of the Y-response, as the responses in each dimension are decoupled (coupled only through  $t_{f}$). 
\begin{table}
\caption{Rendezvous optimal responses when $K^*=1,1.5,2,3$ and $>3$.}
\label{table:draglift1}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline 
$K^*$ & terminal $v_x$ & position & velocity & acceleration\tabularnewline
\hline 
\hline 
~~~1  & $v_{xf}\neq0$ & linear, with $x(t_{f})=0$ & constant, such that $v_{x}(t_{f})\neq0$ & zero\tabularnewline
\hline 
~~~2 & $v_{xf}=0$ & quadratic, with x($t_{f})=0$ & linear & constant \tabularnewline
\hline 
~~~3  & $v_{xf}=0$ & cubic,  x($t_{f})=0$ & quadratic, $v_{x}(t_{f})=0$   & linear, $\dot{v}_{x}(t_{f})=0$ \tabularnewline
\hline 
$>$ 3 & $v_{xf}=0$ & cubic,  x($t_{f})=0$ & quadratic,  $v_{x}(t_{f})=0$  & linear, $\dot{v}_{x}(t_{f})\neq0$\tabularnewline
\hline
\hline
~1.5 & $v_{xf}=v_{x0}\neq0$ & cubic, $x(t_{f})=0$ & quadratic,~$v_{y0}=v_{x0}$,$v_{yf}=-v_{y0}$  & linear %Intercept case,~~$v_{y}(0)=\sqrt{3}v_{x}(0)$ &  
\tabularnewline
%1.5 & cubic, $C_I=0$, $x(t_{f})=0$ & Intercept case,~~$v_{y}(0)=\sqrt{3}v_{x}(0)$ &  
%\tabularnewline
& (2D, $C_I=0)$ &  &  Max initial heading, $\theta_{MAX}=45 ~deg$ &
\tabularnewline
\hline
~1.5 & $v_{xf}=v_{x0}\neq0$ & cubic $x(t_{f})=0$ & quadratic, ~$v_{y0}=\sqrt{3}v_{x0}$,$v_{yf}=+v_{y0}$ & linear %Intercept case,~~$v_{y}(0)=\sqrt{3}v_{x}(0)$ &  
\tabularnewline
%1.5 & cubic, $C_I=0$, $x(t_{f})=0$ & Intercept case,~~$v_{y}(0)=\sqrt{3}v_{x}(0)$ &  
%\tabularnewline
& (2D, $C_I=0)$ &  & Max initial heading, $\theta_{MAX}=30 ~deg$  & \tabularnewline
\hline
\end{tabular}
\end{table}
\begin{figure}[t]
\noindent \begin{centering}
\includegraphics[scale=0.48]{figs/Br_physical}
\par\end{centering}
\noindent \centering{}\caption{Accelerations (red), velocities (blue) and positions (black) for 4 cases of $t_f=Kt_{r}$ and $v_{xf}=0$.}
\label{Figure3}
\end{figure}
It has already been proved that the general depressed quartic polynomial in (\ref{polynomial}) has always at least one positive real root \cite{DSouza1997}, \cite{Carvalho2018}.
However, in the particular case of $C_I=0$, then the quartic polynomial becomes a second order polynomial that may not admit a positive real root in some cases.
The existence of a feasible solution for this minimum energy problem $(C_I=0)$ is discussed in \cite{Guo2019} where a trade-off cost function is introduced in the ZEM/ZEV approach for orbital intercept/rendezvous.
In that work the Hamiltonian equation is very similar to (\ref{eq:Ham}) with the gravity vector in place of the wind acceleration vector.
According to the authors in \cite{Guo2019}, one possible explanation for the inexistence of fine solutions for $t_f$ is that with $C_I=0$ the terminal time is neither constrained nor penalized.
% and, in this way, a longer $t_f$ yields a smaller cost-to-go, and no finite $t_f$ would minimize the %integral of energy. %Also, the authors considers this an "interesting subject for further study".
%Although this makes sense,
This does not however explain why there are some cases in which  $C_I=0$ yields a finite positive terminal time, as we show in this section. 
%In other words, in some situations, there exists indeed a finite $t_f$ minimizing the integral of control %energy.
Aiming at a better understanding of the solutions for the optimal flight time we investigate in this section two special cases under a constant wind.

Consider the problem, shown in Figure \ref{nine}, for a 2D path, with $y_0=0$, $C_I=0$ and ${\bf k=0}$,  for both rendezvous/intercept, where one wants to find the maximum initial heading $\theta$ for which a finite terminal time $t_f$ exists. For the rendezvous, we assume $v_{gxf}=v_{gx0}, v_{gyf}=-v_{gy0}$. For the intercept the terminal velocities  are free at the target. The problem can be transformed into one that searches for the maximum  allowable $v_{y0}$, for a given $v_{x0}$.

\begin{figure}[t]
\noindent \begin{centering}
\includegraphics[scale=0.60]{figs/AIAA_fig_wind_heading.png}
\par\end{centering}
\noindent \centering{}\caption{{Search for the maximum initial heading $\theta$, with $C_I=0$, to obtain a finite optimal $t_f$ solution.}}
\label{nine}
\end{figure}

The corresponding polynomials using ${\bf r}_f=0$ and expressions (\ref{polynomialwzero}) and (\ref{eq:poly_Inter}) are, respectively,
%\begin{equation}
%\begin{array}{l}
%  \mbox{Rendezvous}~~~~~   P(t_{f})=2C_{I}t_{f}^{4}-4(3v_{gx0}^{2}+v_{gy0}^{2})t_{f}^{2}-48{\bf r_{0}}^{T}{\bf v}_{g0}t_{f}-36{\bf r_{0}}{}^{T}{\bf r_{0}} \\
%    \mbox{Intercept}~~~~~~~~~~
%P(t_{f})=2C_{I}t_{f}^{4}-3{\bf v}_{g0}{}^{T}{\bf v}_{g0}t_{f}^{2}-12{\bf r_{0}}^{T}{\bf v}_{g0}t_{f}-9{\bf r_{0}}{}^{T}{\bf r_{0}} \\
%\end{array}
%\end{equation}

%Which, with the given initial/terminal velocities, can be rewritten as:
\begin{eqnarray}
 \mbox{Rendezvous}~     
P(t_{f}) =& C_It_{f}^{4}-2(3v_{gx0}^{2}+v_{gy0}^{2})t_{f}^{2}-24x_{0}v_{gx0}t_{f}-18x_{0}^{2} \\
  \mbox{Intercept}~
P(t_{f}) =& C_{I}t_{f}^{4}-\frac{3}{2}(v_{gx0}^{2}+v_{gy0}^{2})t_{f}^{2}-6x_{0}v_{gx0}t_{f}-\frac{9}{2}x_{0}^{2}~~~ 
\end{eqnarray}
\indent If we consider $C_I=0$, then both polynomials will be very similar. Indeed if we write the terminal time $t_f$ as a function of the reference time (Table 1), or $t_{f}=Kt_{r}=K\left( -\frac{x_{0}}{v_{xg0}} \right)$, then the critical (double) root, for which the discrimant of the quadratic polynomial is zero corresponds  to $K=1.5$ (in both cases), or $t_{f}=-1.5\dfrac{x_{g0}}{v_{xg0}}$:

\begin{equation}
\begin{array}{c}
      P(K)=(\alpha_0) K^{2}-12K-9=0  \\ 
  
   \mbox{~~Rendezvous} ~~~~~~~~~~~~~~~~~~~~~~~~~~\mbox{~~~ ~~~Intercept}\\
   
   \alpha_0=\left( \dfrac{-3( v_{gx0}^{2}+\frac{1}{3}v_{gy0}^{2})}{v_{gx0}^{2} }\right)=4 ~~~~~~
   \alpha_0=\left(\dfrac{-3(v_{gx0}^{2}+v_{gy0}^{2})}{v_{gx0}^{2}}\right)=4  \\
\end{array}
\end{equation}

Nevertheless, the critical orthogonal velocity, and the maximum initial heading are different for each case:

\begin{eqnarray}
 \mbox{Rendezvous}~
v_{{gy0}_{MAX}}=& v_{gx0}~~~~\theta_{MAX}=45~ deg \\ 
  \mbox{Intercept}~
v_{{gy0}_{MAX}}=&\dfrac{v_{gx0}}{\sqrt{3}}~~~~\theta_{MAX}=30 ~deg
\end{eqnarray}

The heading limitation ($30 ~deg$) for the intercept problem is in agreement with the results of \cite{Hawking2013}, although there was no analysis performed for the rendezvous case in that reference. Note also that in  \cite{Bakolas2014} a minimum-time problem is solved and there is no initial heading constraint for the optimal intercept.

A plot of the optimal $K$-parameter (multiple of the reference time) as function of the velocity $v_{gy0}$ is shown on the right side of Figure \ref{10} for $x_0=3,v_{gx0}=-1$ and for both the rendezvous and the intercept scenarios.
\begin{figure}[t]
\noindent \begin{centering}
\includegraphics[scale=0.68]{figs/roots_intercept2b.png}
\par\end{centering}
\noindent \centering{}\caption{{Roots of time-optimal polynomial as a function of $v_{gyo}$, with $C_I=1e^{-6},x_0=3,v_{gx0}=-1.$}}
\label{10}
\end{figure}
If instead of considering a quadratic polynomial (with $C_I=0$) one would consider the original quartic polynomials with a very small $C_I$, then we would obtain the plot of the $K$-parameter as shown on the left side of Figure \ref{10}. Note that the figure shows only the three positive real roots of the polynomial (as the fourth one is negative).
Notice also that there is always a large time solution as $t_f \to \infty$ for $C_I \to 0$. This slow time response is the solution for the minimum-energy problem commented in \cite{Guo2019}, which will always exist for any problem with $C_I \to 0$. 
However, in some cases, there will still be two other local optimal time solutions. Indeed, this behavior in the multiple roots of a polynomial is known as "bifurcation" and was referred to in  \cite{Bakolas2014} for an intercept problem as "jump solutions" or "manifold discontinuities". Note also that, although the intercept guidance in \cite{Bakolas2014} does not show heading constraints, it still may exhibit "jump solutions" corresponding to the value of the K-parameter for which the number of positive real roots of $P(t_f)$ changes from three to one.


\iffalse
\begin{table}
\caption{Cases of time-optimal polynomial $P(t_f)$}
\label{table:tablepoly}
\centering
\begin{tabular}{|c|c|c|c|}
\hline 
 Case & ${\bf v}_g(t_f)$  & $\frac{dw}{dt}$ & Polynomial $P(t_{f})$
 \tabularnewline
\hline 
\hline 
1 (R) & ${\bf 0}$ & ${\bf 0}$ & $C_{I}t_{f}^{4}-2({\bf v}_{g0}^{T}{\bf v}_{g0})t_{f}^{2}-12({\bf r_{0}}^{T}{\bf v}_{g0})t_{f}-18({\bf r_{0}}{}^{T}{\bf r_{0}})$
\tabularnewline
\hline 
2 (R) & ${\bf 0}$ & ${\bf {k}}$ &
$(2C_{I}+{\bf k}^{T}{\bf k})t_{f}^{4}-4({\bf v}_{g0}^{T}{\bf v}_{g0})t_{f}^{2}-24({\bf r_{0}}^{T}{\bf v}_{g0})t_{f}-36({\bf r_{0}}{}^{T}{\bf r_{0}})$
\tabularnewline
\hline 
3 (R) & ${\bf v}_{gf}$ & ${\bf \overline{k}}$ &
$(2C_{I}+{\bf \overline{k}}^{T}{\bf \overline{k}})t_{f}^{4}-4({\bf v}_{g0}{}^{T}{\bf v}_{g0}+{\bf v}_{gf}{}^{T}{\bf v}_{gf}+{\bf v}_{gf}^{T}{\bf v}_{g0})t_{f}^{2}-24{\bf r_{0}}^{T}({\bf v}_{g0}+{\bf v}_{gf})t_{f}-36{\bf r_{0}}{}^{T}{\bf r_{0}}$
\tabularnewline
\hline 
4 (R) & $[{\bf v}_{gx0},-{\bf v}_{gy0}]$
& ${\bf \overline{k}}$ &
$(2C_{I}+{\bf \overline{k}}^{T}{\bf \overline{k}})t_{f}^{4}-4(3v_{gx0}^{2}+v_{gy0}^{2})t_{f}^{2}-48{\bf r_{0}}^{T}{\bf v}_{g0}t_{f}-36{\bf r_{0}}{}^{T}{\bf r_{0}} $
\tabularnewline
\hline 
5 (R) & $[{\bf v}_{gx0},{\bf v}_{gy0}]$
& ${\bf \overline{k}}$ &
$(2C_{I}+{\bf \overline{k}}^{T}{\bf \overline{k}})t_{f}^{4}-12(v_{gx0}^{2}+v_{gy0}^{2})t_{f}^{2}-48{\bf r_{0}}^{T}{\bf v}_{g0}t_{f}-36{\bf r_{0}}{}^{T}{\bf r_{0}} $
\tabularnewline
\hline 
6 (I) &  free & ${\bf {k}}$ &
$(2C_{I}+\frac{3}{4}{\bf k}^{T}{\bf k})t_{f}^{4}-3({\bf v}_{g0}{}^{T}{\bf v}_{g0}+{\bf r_{0}}^{T}{\bf k})t_{f}^{2}-12{\bf r_{0}}^{T}{\bf v}_{g0}t_{f}-9{\bf r_{0}}{}^{T}{\bf r_{0}}$
\tabularnewline
\hline 
7 (I) & free &  ${\bf {0}}$ &
$2C_{I}t_{f}^{4}-3{\bf v}_{g0}{}^{T}{\bf v}_{g0}t_{f}^{2}-12{\bf r_{0}}^{T}{\bf v}_{g0}t_{f}-9{\bf r_{0}}{}^{T}{\bf r_{0}}$
\tabularnewline
\hline 
\end{tabular}
\end{table}
\fi


%It is interesting to note that, for a constant wind condition (${\bf k=0})$ and a minimum-energy problem $(C_{I}\to0),$ this quartic polynomial will be reduced to a 2nd order polynomial, which yields a positive real root only if $|v_{gy0}|\leq|v_{gx0}|,$ corresponding to an initial heading angle, toward the target, lesser than 45 deg. However, the inclusion of a trade-off paramenter $C_{I}\neq0$, or even the presence of a wind gradient ${\bf k \neq0}$, will withdraw this initial heading constraint, assuring at least one positive real root for the quartic polynomial, independent of the initial heading.



==> intercept.tex <==
\section{Problem solution: intercept case}
\label{six}




==> rendezvous.tex <==
\section{Case studies for particular wind speed/accelerations}
\label{sec:rendezvous}

Here we analyse the optimal acceleration and the optimal terminal
time, corresponding to the solution of the rendezvous guidance problem
(\ref{eq:statement}), for three particular wind conditions, that are:
\begin{enumerate}
\item Constant wind speed, with null terminal velocity.
\item Constant wind speed rate (or wind acceleration).
\item Constant wind speed gradient in the cross-track direction.
\end{enumerate}

The case of piecewise linear wind speed may be of practical
interest, as it can be used to treat the more general wind field cases of a vehicle in
a spatio-temporal flow field with wind shear parameters \cite{2001Airplane},\cite{Bakolas2018}.

\subsection{Case - constant wind and null terminal velocity}


Note that, in the absence of wind, or even in a constant
wind, we have $\Delta_{{\bf w}}(t_{f})={\bf 0},\,\,{\bf \varpi}(t_{f})={\bf 0}$
from (\ref{eq:deltaOmega}).
\begin{figure}[hbtp]
\noindent \begin{centering}
\includegraphics[scale=0.60]{figs/AIAA_fig_wind_cnst.png}
\par\end{centering}
\noindent \centering{}\caption{{Optimal problem (time-energy) for a UAV in constant wind speed.}}
\end{figure}

Then, assuming the target in the
origin (${\bf r_{f}}=0$) and a null final velocity (${\bf v}_{gf}={\bf 0}$), and using the methodology presented in the previous section, we have the  optimal costates, acceleration and terminal Hamiltonian equation as:
\begin{equation}
\begin{array}{ccc}
{\bf {\bf p}}_{r}=6\dfrac{\left[2{\bf r_{0}}+{\bf v}_{g0}t_{f}\right]}{t_{f}^{3}} & \,\,\,\,\,\,\,\,\,\,\,\,\,\, & {\bf {\bf p}}_{v}(0)=\dfrac{2\left[3{\bf r_{0}}+2{\bf v}_{g0}t_{f}\right]}{t_{f}^{2}}\end{array}\label{eq:JVD-1-1-1}
\end{equation}
%As well as the resulting linear equation for the optimal acceleration,
%from (\ref{eq:optacel}), as
\begin{equation}
{\bf u}^{*}(t)=t{\bf {\bf p}}_{r}-{\bf p}_{v}(0)=6t\dfrac{\left[2{\bf r_{0}}+{\bf v}_{g0}t_{f}\right]}{t_{f}^{3}}-\dfrac{2\left[3{\bf r_{0}}+2{\bf v}_{g0}t_{f}\right]}{t_{f}^{2}}\label{eq:optbruno}
\end{equation}
%Thus, the terminal acceleration ${\bf u}^{*}(t_{f})$ is equal to
%\begin{equation}
%{\bf u}^{*}(t_{f})=\dfrac{\left[6{\bf r_{0}}+2{\bf v}_{g0}t_{f}\right]}{t_{f}^{2}}\label{eq:optbr}
%\end{equation}
%And now, we can find the optimal terminal time $t_{f}^{*}$ for the optimization
%problem in (\ref{eq:statement}), using the Hamiltonian equation (\ref{eq:Hamil})
%evaluated at $t_{f}$, recalling that ${\bf v}_{g}(t_{f})={\bf 0}$, in this particular case, that is:
\begin{equation}
\begin{array}{c}
H(t_{f})=0\,\Rightarrow{\bf u}^{*T}(t_{f})\left[{\bf u}^{*}(t_{f})+2 \dot{ \bf w}(t_{f})\right]=2\left[C_{I}+{\bf p}_{r}^{T}{\bf v}_{g}(t_{f})\right]\\
{\bf \Rightarrow u}^{*T}(t_{f}){\bf u}^{*}(t_{f})=2C_{I}\\
\left[6{\bf r_{0}}+2{\bf v}_{g0}t_{f}\right]^{T}\left[6{\bf r_{0}}+2{\bf v}_{g0}t_{f}\right]=2C_{I}t_{f}^{4}
\end{array}\label{eq:z}
\end{equation}
Yielding the 4th order time-optimal polynomial $P(t_{f})$ as
\[
P(t_{f})=2C_{I}t_{f}^{4}-4({\bf v}_{g0}^{T}{\bf v}_{g0})t_{f}^{2}-24({\bf r_{0}}^{T}{\bf v}_{g0})t_{f}-36({\bf r_{0}}{}^{T}{\bf r_{0}})=0
\]
which is the same depressed quartic polynomial appearing in \cite{DSouza1997}  and \cite{Carvalho2018}, where the wind is not considered. Obviously, under a constant wind, the relative
airspeed rate and the inertial velocity rate are exactly the same.

\subsection{Case - constant wind acceleration}

Now, we consider the case of a constant rate of the wind speed, $\dot{ \bf w}(t)={\bf k}$,
which means that the wind, in a given direction, 
is increasing ($k>0$) or decreasing ($k<0$) linearly with time. We
also suppose here that the terminal velocity ${\bf v}_{g}(t_f)$ may be
constrained to any desired value. 
%In the following, we will find the
%optimal acceleration expression, as well as the optimal terminal time %$t_{f}^{*}.$ 
\begin{figure}[hbtp]
\noindent \begin{centering}
\includegraphics[scale=0.60]{figs/AIAA_fig_wind_incr1.png}
\par\end{centering}
\noindent \centering{}\caption{{Optimal problem (time-energy) for a UAV in linearly time-varying wind
speed.}}
\end{figure}
First, let us compute $\Delta_{{\bf w}}(t_{f})$ and ${\bf \varpi}(t_{f})$
for this case, from (\ref{eq:deltaOmega}), as:
\begin{equation}
\begin{array}{c}
\Delta_{{\bf w}}(t_{f})=\int_{0}^{t}{ {\dot{\bf w}}}(t)dt={\bf w}(t_{f})-{\bf w}(0)={\bf k}t_{f}\\
{\bf \varpi}(t_{f})=\int_{0}^{t}\int_{0}^{t}{ {\dot{\bf w}}}(t)dtd\tau=\int_{0}^{t_{f}}{\bf w}(t)dt-{\bf w}(0)t_{f}=\frac{{\bf k}t_{f}^{2}}{2}
\end{array}\label{eq:deltaOmega2-1-1}
\end{equation}
Then, assuming
the target position at the origin (${\bf r}_{f}=0$), the corresponding optimal costates, acceleration and terminal Hamiltonian equation, for this case, are:
\[
\begin{array}{c}
{\bf {\bf p}}_{r}=6\dfrac{\left[2{\bf r_{0}}+({\bf v}_{g0}+{\bf v}_{gf})t_{f}-{\bf k}t_{f}^{2}+2\frac{{\bf k}t_{f}^{2}}{2}\right]}{t_{f}^{3}}=6\dfrac{\left[2{\bf r_{0}}+({\bf v}_{g0}+{\bf v}_{gf})t_{f}\right]}{t_{f}^{3}}\\
{\bf {\bf p}}_{v}(0)=\dfrac{2\left[3{\bf r_{0}}+(2{\bf v}_{g0}+{\bf v}_{gf}-{\bf k}t_{f})t_{f}+3\frac{{\bf k}t_{f}^{2}}{2})\right]}{t_{f}^{2}}=\dfrac{2\left[3{\bf r_{0}+}(2{\bf v}_{g0}+{\bf v}_{gf})t_{f}\right]}{t_{f}^{2}}+{\bf k}
\end{array}
\]
%And the resulting linear equation for the optimal airspeed acceleration,
%from (\ref{eq:optacel}), is:
\begin{equation}
{\bf u}^{*}(t)=t{\bf {\bf p}}_{r}-{\bf p}_{v}(0)=6t\dfrac{\left[2{\bf r_{0}}+({\bf v}_{g0}+{\bf v}_{gf})t_{f}\right]}{t_{f}^{3}}-\dfrac{2\left[3{\bf r_{0}+}(2{\bf v}_{g0}+{\bf v}_{gf})t_{f}\right]}{t_{f}^{2}}-{\bf k}\label{eq:acc_comp}
\end{equation}
%With the terminal acceleration ${\bf u}^{*}(t_{f})$ given by
%\begin{equation}
%{\bf u}^{*}(t_{f})=\dfrac{\left[6{\bf r_{0}}+(2{\bf v}_{g0}+4{\bf v}_{gf})t_{f}\right]}{t_{f}^{2}}-{\bf k}\label{eq:acc_comp1}
%\end{equation}
%For the evaluation of $t_f^*$, first recall the Hamiltonian equation
%(\ref{eq:Hamil}), evaluated at the final time, or $H(t_{f})=0:$
\[
\begin{array}{c}
{\bf u}^{*T}(t_{f})\left[{\bf u}^{*}(t_{f})+2{\bf k}\right]=2\left[C_{I}+{\bf p}_{r}^{T}{\bf v}_{gf}\right]\\
\Rightarrow\left[6{\bf r_{0}}+(2{\bf v}_{g0}+4{\bf v}_{gf})t_{f}-{\bf k}t_{f}^{2}\right]^{T}\left[6{\bf r_{0}}+(2{\bf v}_{g0}+4{\bf v}_{gf})t_{f}+{\bf k}t_{f}^{2}\right]=2C_{I}t_{f}^{4}+12{\bf v}_{gf}^{T}\left[2{\bf r_{0}}+({\bf v}_{g0}+{\bf v}_{gf})t_{f}\right]
\end{array}
\]
whose expansion yields the 4th order time-optimal polynomial $P(t_{f})$
as
\begin{equation}
P(t_{f})=(2C_{I}+{\bf k}^{T}{\bf k})t_{f}^{4}
-4({\bf v}_{g0}{}^{T}{\bf v}_{g0}+{\bf v}_{gf}{}^{T}{\bf v}_{gf}+{\bf v}_{gf}^{T}{\bf v}_{g0})t_{f}^{2}
-24{\bf r_{0}}^{T}({\bf v}_{g0}+{\bf v}_{gf})t_{f}-36{\bf r_{0}}{}^{T}{\bf r_{0}}=0
\label{eq:polygeral}
\end{equation}

%where
%\[
%\begin{array}{l}
%a_{4}=\,\,\,2C_{I}+{\bf k}^{T}{\bf k}\\
%a_{3}=\,\,\,0\\
%a_{2}=-4({\bf v}_{g0}+2{\bf v}_{gf}){}^{T}({\bf v}_{g0}+2{\bf %v}_{gf})+12{\bf v}_{gf}^{T}({\bf v}_{g0}+{\bf v}_{gf})=-4({\bf %v}_{g0}{}^{T}{\bf v}_{g0}+{\bf v}_{gf}{}^{T}{\bf v}_{gf}+{\bf %v}_{gf}^{T}{\bf v}_{g0})\\
%a_{1}=-24{\bf r_{0}}^{T}({\bf v}_{g0}+2{\bf v}_{gf})+24{\bf %v}_{gf}^{T}{\bf r_{0}}=-24{\bf r_{0}}^{T}({\bf v}_{g0}+{\bf v}_{gf})\\
%a_{0}=-36{\bf r_{0}}{}^{T}{\bf r_{0}}
%\end{array}
%\]

 Thus, we conclude that a linearly
increasing (or decreasing) wind works as an effective increase in the
trade-off parameter $C_{I}$, yielding a smaller optimal final time
$t_{f},$ when compared to the same equivalent condition without wind
(or with a constant wind).

%It is interesting to note that, in the case of a null terminal velocity
%(${\bf v}_{g}(t_{f})=0$), this optimal time polynomial will be further
%reduced to:
%\[
%P(t_{f})=(2C_{I}+{\bf k}^{T}{\bf k})t_{f}^{4}-4({\bf v}_{g0}^{T}{\bf %v}_{g0})t_{f}^{2}-24({\bf r_{0}}^{T}{\bf v}_{g0})t_{f}-36({\bf %r_{0}}{}^{T}{\bf r_{0}})=0
%\]
%which is the same quartic polynomial appearing in \cite{Carvalho2018}
%and in \cite{DSouza1997}, when the wind is not considered, except by
%the additional term ${\bf k}^{T}{\bf k}$ in the fourth degree %coefficient
%term.

\subsection{Case - constant wind shear in cross-track direction}
Now, we consider the particular case of a wind with a constant
shear (gradient) in the cross-track direction, as in Figure 6. To simplify the analysis, we suppose here a 2D movement. This problem is closely
related to the classical Zermelo problem, for the minimum time navigation
with constant airspeed, and whose solution is analysed with many different optimization approaches
in the literature \cite{2001Airplane}, [Lewisbook].
\begin{figure}[hbtp]
\noindent \begin{centering}
\includegraphics[scale=0.60]{figs/AIAA_fig_wind_shear.png}
\par\end{centering}
\noindent \centering{}\caption{{Optimal problem (time-energy) for a UAV in constant wind shear in
cross-track direction. }}
\end{figure}
In this case, the wind speed in the along-track direction ($x$) is supposed to vary linearly with the cros-track direction ($y$), such that the vertical wind speed component
will be always null ($w_{y}=0$), while the horizontal wind  will be given by $w_{x}=ky(t)$, or in matricial form:
\[
{\bf {w}}(t)={\bf Kr}
\]
where ${\bf K}=\left[\begin{array}{cc}
0 & k\\
0 & 0
\end{array}\right]_{2\times2}$ and ${\bf r}=[x~~y]^T.$ Such that the wind speed rate is
\[
 \dot{\bf {w}}(t)= {\bf K}\dot{\bf r}={\bf Kv}_{g}(t)
\]

The Hamiltonian function for this problem, using (\ref{eq:Ham}),
is given by
\begin{equation}
\begin{array}{c}
%H=C_{I}+\frac{1}{2}{\bf u}^{T}{\bf u}+{\bf p}_{r}^{T}{\bf v}_{g}+{\bf p}_{v}^{T}( \dot{\bf w}+{\bf u})\\
H=C_{I}+\frac{1}{2}{\bf u}^{T}{\bf u}+{\bf p}_{r}^{T}{\bf v}_{g}+{\bf p}_{v}^{T}({\bf {\bf Kv}_{g}+u})
\label{eq:hamilshear}
\end{array}
\end{equation}
where ${\bf p}_{r}$ and ${\bf p}_{v}$ are the costate vectors associated
with the position and velocity vectors, respectively, such that:
%A necessary
%condition for optimality is $H_{{\bf u}}=\frac{\partial H}{\partial{\bf u}}=0$,
%which yields
\[
{\bf u^{*}}= \dot{\bf v}_{a}^{*}=-{\bf p}_{v}\label{eq:ustar-1}
\]

To derive the costate vectors, we first rewrite the Hamiltonian equation as
\begin{equation}
\begin{array}{c}
%H=C_{I}+\frac{1}{2}{\bf u}^{T}{\bf u}+{\bf p}_{r}^{T}{\bf v}_{g}+{\bf p}_{v}^{T}( \dot{\bf w}+{\bf u})\\
H=C_{I}-\frac{1}{2}{\bf u}^{T}{\bf u}+{\bf p}_{r}^{T}{\bf v}_{g}+{\bf p}_{v}^{T}{\bf {\bf Kv}_{g}}
\label{eq:hamilshear}
\end{array}
\end{equation}

Such that according to PMP and Hamilton's, the costate equations are obtained as:
\[
\begin{array}{c}
{\dot{\bf  p}}_{r}=-\dfrac{\partial H}{\partial{\bf r}}={\bf 0}
\\
{ \dot{\bf p}}_{v}=\dfrac{\partial H}{\partial{\bf v_{g}}}=
\dfrac{\partial \{\frac{1}{2}{\bf u}^{T}{\bf u}\}}{\partial{\bf u}}
-{\bf p}_{r}-{\bf {\bf K}}^{T}{\bf p}_{v}=
{\bf u} \dfrac{\partial {\bf u}}{\partial{\bf v_{g}}}
{\bf -{\bf p}}_{r}-{\bf {\bf K}}^{T}{\bf p}_{v}=
{\bf {\bf K}}^{T}{\bf p}_{v}-{\bf p}_{r}-{\bf {\bf K}}^{T}{\bf p}_{v}
=-{\bf p}_{r}
\end{array}
\]

Whose solution comes to:

\[
{\bf u^{*}}=\dot{\bf  v}_{a}^{*}=-\left[\begin{array}{l}
p_{vx}\\
p_{vy}
\end{array}\right]=\left[\begin{array}{l}
tp_{rx}-p_{vx}(0)\\
tp_{ry}-p_{vy}(0)
\end{array}\right]
\]

%and the optimal inertial acceleration will be:
%\begin{equation}
% \dot{\bf v}_{g}^{*}={\bf u}^{*}+ \dot{\bf w}(t)={\bf u}^{*}+{\bf Kv}_{g}\label{eq:acel1-1}
%\end{equation}

As well as the optimal inertial acceleration:
\begin{equation}
\dot{\bf  v}_{g}^{*}=
\dot{\bf  v}_{a}^{*}
+ {\bf Kv}_{g}
=\left[\begin{array}{l}
tp_{rx}-p_{vx}(0)\\
tp_{ry}-p_{vy}(0)
\end{array}\right]
+
\left[\begin{array}{l}
kv_{gy}(t)\\
0
\end{array}\right]
\label{vgak}
\end{equation}


%Or 
%\begin{equation}
%\begin{array}{l}
%{ { {\dot{\bf v}}_{g}^{*}}=}\left[\begin{array}{l}
%\dot{v}_{gx}\\
%\dot{v}_{gy}
%\end{array}\right]=\left[\begin{array}{l}
%t(p_{rx}+kp_{vy}(0))-\frac{t^{2}}{2}kp_{ry}-p_{vx}(0)\\
%tp_{ry}-p_{vy}(0)
%\end{array}\right]+k\left[\begin{array}{l}
%\frac{t^{2}}{2}p_{ry}-tp_{vy}(0)+v_{gy0}\\
%0
%\end{array}\right]\\ \\
%{ { {\dot{\bf v}}_{g}^{*}}=}\left[\begin{array}{l}
%\dot{v}_{gx}\\
%\dot{v}_{gy}
%\end{array}\right]=\left[\begin{array}{l}
%tp_{rx}-p_{vx}(0)\textcolor{red}{+kv_{gy0}}\\
%tp_{ry}-p_{vy}(0)
%\end{array}\right]
%=
%t{ {\bf p}}_{r}-{{\bf p}}_{v}(0)+
%\left[\begin{array}{l}
%\textcolor{red}{kv_{gy0}}\\
%0
%\end{array}\right]
%\end{array}
%\label{vgoptimal}
%\end{equation}
%Where the new term is highlighted in red.

Whose integration produces the expressions for the inertial positions/velocities components

\[
\begin{array}{ccc}
\left\{ \begin{array}{l}
v_{gx}(t)=\frac{t^{2}}{2}p_{rx}-tp_{vx0}{+k{y}}(t)+v_{gx0}\\
x(t)=\frac{t^{3}}{6}p_{rx}-\frac{t^{2}}{2}p_{vx0}{+k}
\int_0^t y(t)
+tv_{gx0}+x_{0}
\end{array}\right. & & 

\left\{ \begin{array}{l}
v_{gy}(t)=\frac{t^{2}}{2}p_{ry}-tp_{vy0}+v_{gy0}\\
y(t)=\frac{t^{3}}{6}p_{ry}-\frac{t^{2}}{2}p_{vy0}+tv_{gy0}+y_{0}
\end{array}\right.
\end{array}
\]

Or
\[
\begin{array}{ccc}
\left\{ \begin{array}{l}
v_{gx}(t)=\frac{t^{2}}{2}p_{rx}-tp_{vx0}+k
(\frac{t^{3}}{6}p_{ry}-\frac{t^{2}}{2}p_{vy0}+tv_{gy0})
+v_{gx0}\\
x(t)=\frac{t^{3}}{6}p_{rx}-\frac{t^{2}}{2}p_{vx0}{+k}
(\frac{t^{4}}{24}p_{ry}-\frac{t^{3}}{6}p_{vy0}+\frac{t^{2}}{2}v_{gy0})
+tv_{gx0}+x_{0}
\end{array}\right. & & 

\left\{ \begin{array}{l}
v_{gy}(t)=\frac{t^{2}}{2}p_{ry}-tp_{vy0}+v_{gy0}\\
y(t)=\frac{t^{3}}{6}p_{ry}-\frac{t^{2}}{2}p_{vy0}+tv_{gy0}+y_{0}
\end{array}\right.
\end{array}
\]
Using these equations, and recalling the particular initial/terminal conditions (Fig. 6), where  $v_{xf}=v_{x0}$, $v_{yf}=-v_{y0}$, we can find the optimal costate vectors as: 
\[
\begin{array}{ccc}
{\bf {\bf p}}_{r}=\left[\begin{array}{c}
\frac{12}{t_f^{3}}(x_{0}+v_{gx0}t_{f}){+\frac{2}{t_f}kv_{gy0}}\\
0
\end{array}\right]
& & 
{\bf {\bf p}}_{v}(0)=\left[\begin{array}{c}
\frac{6}{t_f^{2}}(x_{0}+v_{gx0}t_{f}){+kv_{gy0}}\\
\frac{2}{t_f}v_{gy0}
\end{array}\right]
\end{array}
\]

Such that the initial/terminal inertial accelerations, from (\ref{vgak}), are written as
\[
\begin{array}{l}
{ { {\dot{\bf v}}_{g}^{*}}}(t_f)=t_f{ {\bf p}}_{r}-{{\bf p}}_{v}(0)
+
\left[\begin{array}{c}
-{kv_{gy0}}\\
0
\end{array}\right]
=
\dfrac{1}{t_{f}^{2}}\left[6{\bf r_{0}}+(2 {\bf v}_{g0} +4 {\bf v}_{gf})t_{f}\right]
 \\
{ { {\dot{\bf v}}_{g}^{*}}}(0)=-{{\bf p}}_{v}(0)+
\left[\begin{array}{c}
{kv_{gy0}}\\
0
\end{array}\right] =
-\dfrac{1}{t_{f}^{2}}\left[6{\bf r_{0}}+(4 {\bf v}_{g0} +2 {\bf v}_{gf})t_{f}\right]
\end{array}
\]

At a first glance, it may seem that the optimal inertial accelerations do not depend on the wind, as ${\bf v}_{g}(t_{f})$ do not depend on the $k$ parameter. However, this happens only for the terminal value of ${\bf v}_{g}(t)$. Moreover, the wind influence will also appear through the optimal terminal time $t_f$, as this is also dependent on $k$, as will be shown in the sequel.

The terminal relative acceleration is then written as:
\[
\begin{array}{l}
{\bf u}^{*}(t_f)=
t_f{ {\bf p}}_{r}-{{\bf p}}_{v}(0)=
\left[\begin{array}{c}
\frac{6}{t_f^{2}}(x_{0}+v_{gx0}t_{f})+kv_{gy0}\\
-\frac{2}{t_f^{2}}v_{gy0}t_{f}
\end{array}
\right]
%{\bf u}^{*}(0)={ { {\dot{\bf v}}_{g}^{*}}}(0)-\dot{\bf w}(0)=
%-\dfrac{1}{t_{f}^{2}}\left[6{\bf r_{0}}+(4 {\bf v}_{g0} +2 {\bf v}_{gf})t_{f}\right]
%-\left[\begin{array}{c}
%{kv_{gy0}}\\
%0
%\end{array}\right]
\end{array}
\]

%Another way to come to the same result is to combine (\ref{eq:acel1-1}) and (\ref{vgoptimal}) to yield
%\begin{equation}
% {\bf u}^{*}(t)=\dot{\bf v}_{g}^{*}(t)-\dot{\bf w}(t)
% =
% \left[\begin{array}{l}
%tp_{rx}-p_{vx}(0){-k(v_{gy}(t)-v_{gy0})}\\
%tp_{ry}-p_{vy}(0)
%\end{array}\right]
%\label{eq:acel1-12}
%\end{equation}


%Then, the terminal acceleration is finally given by
 %\[
%{ \bf u}^{*}(t_f)=\left[\begin{array}{l}
%u_{xf}^*\\
%u_{yf}^*
%\end{array}\right]\\
 %\]
 
Such that the equation for the terminal Hamiltonian, $H(t_{f})$=0, is given by:
\begin{equation}
{\bf u}^{*T}(t_{f})\left[{\bf u}^{*}(t_{f})+2{\bf Kv}_{g}(t_f)\right]=2\left[C_{I}+{\bf p}_{r}^{T}{\bf v}_{g}(t_{f})\right]\label{eq:Hamil-1}
\end{equation}

Resulting in the following equation:
\[
\left[\begin{array}{c}
\frac{6}{t_f^{2}}(x_{0}+v_{gx0}t_{f})+kv_{gy0}\\
-\frac{2}{t_f}v_{gy0}
\end{array}
\right]^T
\left[\begin{array}{c}
\frac{6}{t_f^{2}}(x_{0}+v_{gx0}t_{f})-kv_{gy0}\\
-\frac{2}{t_f}v_{gy0}
\end{array}
\right]
=
2C_I+\frac{24v_{gx0}}{t_f^{3}}(x_{0}+v_{gx0}t_{f})+{\frac{4}{t_f}kv_{gx0}v_{gy0}}
 \]

%where we have used the definition ${\bf \overline{k}}=[
%-2kv_{gy}(t_{f}),~~
%0]^T$.

The expansion of this equation yields the 4th order time-optimal polynomial $P(t_{f})$
as
\begin{equation}
P(t_{f})=(2C_{I}+k^2{v}_{gy0}^2)t_{f}^{4}+({4kv_{gx0}v_{gy0}})t_{f}^{3} -4(3{v}_{gx0}^2+{v}_{gy0}^2)t_{f}^{2}-48 x_{0}{v}_{gx0}t_{f}-36x_{0}^2=0
\label{eq:poly_rd2}
\end{equation}

%where
%\[
%\begin{array}{l}
%a_{4}=\\
%a_{3}=0\\
%a_{2}=-12{v}_{gx0}^2-4{v}_{gy0}^2\\
%a_{1}=-48 x_{0}{v}_{gx0}\\
%a_{0}=-36x_{0}^2
%\end{array}
%\]

%Notice that the term $k^2{v}_{gy0}^2$ increases the equivalent trade-off parameter $C_I$, reducing the  travel time.
%Also, the time polynomial will yield the same optimal terminal time, independent of the signal of $k$. Such that the difference will appear in the optimal control $u^*$, with higher airspeeds and cost-to-go for increasing heading winds as opposed to the increasing tail winds case. 


\subsection{Case - constant wind shear in cross-track direction and CONSTANT airspeed}

We consider the previous case of constant wind shear but now trying to impose a constant airspeed during the whole travel.
A first approach, that generates a simple solution, is to find the optimal terminal time for which the airspeed at the middle of the path is equal to the initial airspeed.

In this particular position, the lateral airspeed is null, or $v_{ay}=0$ and the longitudinal airspeed is given by $v_{ax}(t)=v_{gx}(t)-ky(t)$. Such that the imposition of the same airspeed in $t=0$ and $t=t_f$ gives:

\[
v_{ax}(\frac{t_f}{2})=v_{gx}(\frac{t_f}{2})-ky(\frac{t_f}{2})= \sqrt{v_{gx0}^2+v_{gy0}^2}=V_{a0}
\]

Indeed, using the optimal costates from the previous section, we can write the longitudinal airspeed as

\[
\begin{array}{l}
v_{ax}(t)=\frac{t^{2}}{2}p_{rx}-tp_{vx0}
+v_{gx0}\\
v_{ax}(t)=
(\frac{t^{2}}{t_f}-t)p_{vx0}+v_{gx0}\\
\end{array}
\]

And for $t=\frac{t_f}{2}$, we have

\[
\begin{array}{l}
v_{ax}(\frac{t_f}{2})=V_{a0}=-\frac{t_f}{4}p_{vx0}+v_{gx0}\\
V_{a0}=-\frac{t_f}{4}
( \frac{6}{t_f^{2}}(x_{0}+v_{gx0}t_{f})+kv_{gy0})+v_{gx0}\\
V_{a0}=
-\frac{t_f}{4t_f^2}
( 6(x_{0}+v_{gx0}t_{f})+kv_{gy0}t_f^2) -4v_{gx0}t_f )\\
V_{a0}=
-\frac{1}{4t_f}
( 6(x_{0}+v_{gx0}t_{f})+kv_{gy0}t_f^2) -4v_{gx0}t_f )
\end{array}
\]

Resulting in the simple second order equation that yields the optimal terminal time $t_f$ for a constant airspeed case:
\[
P(t_f)=
-kv_{gy0}t_f^2 -(2v_{gx0}+4V_{a0})t_{f} -6x_{0}=0
\]

